MoA: Mixture-of-Attention for Subject-Context Disentanglement in Personalized Image Generation

We introduce a new architecture for personalization of text-to-image diffusion models, coined Mixture-of-Attention (MoA). Inspired by the Mixture-of-Experts mechanism utilized in large language models (LLMs), MoA distributes the generation workload between two attention pathways: a personalized branch and a non-personalized prior branch. MoA is designed to retain the original model's prior by fixing its attention layers in the prior branch, while minimally intervening in the generation process with the personalized branch that learns to embed subjects in the layout and context generated by the prior branch. A novel routing mechanism manages the distribution of pixels in each layer across these branches to optimize the blend of personalized and generic content creation. Once trained, MoA facilitates the creation of high-quality, personalized images featuring multiple subjects with compositions and interactions as diverse as those generated by the original model. Crucially, MoA enhances the distinction between the model's pre-existing capability and the newly augmented personalized intervention, thereby offering a more disentangled subject-context control that was previously unattainable. Project page: https://snap-research.github.io/mixture-of-attention

==> table/ablation.tex <==
\begin{table}[t]  \centering
	\small
	\caption{Ablation.}
	\vspace{-0.4cm}
	\label{table1}
	\begin{tabular}{c|cc|ccl}
		\bottomrule
		\multirow{2}{*}{\textbf{Methods}} & \multicolumn{2}{c|}{\textit{\textbf{Single-Subject}}} & \multicolumn{2}{c}{\textit{\textbf{Multi-Subject}}} \\
		& IP  $\uparrow$       & PC $\uparrow$     &IP $\uparrow$      & \multicolumn{2}{c}{PC $\uparrow$}     \\
		\midrule
          \textbf{Mixture-of-Attention} (full)                & -   & -        & -         & \multicolumn{2}{c}{ - }     \\
          \midrule
          - MoA \\
          - NeTI \\
          - Maximum training step \\
          
  
	\end{tabular} \\
	\label{table:ablation}
\end{table}



==> table/comparison.tex <==
\begin{table}[t]  \centering
	\small
	\caption{Quantitative results for all competing methods on single- and multi-subject generation. IP denotes identity preservation and PC denotes prompt consistency. OF stands for ``optimization-free'' inference.}
	\vspace{-0.4cm}
	\label{table1}
	\begin{tabular}{cc|cc|ccl}
		\bottomrule
		\multirow{2}{*}{\textbf{Methods}} & & \multicolumn{2}{c|}{\textit{\textbf{Single-Subject}}} & \multicolumn{2}{c}{\textit{\textbf{Multi-Subject}}} \\
		& OF & IP  $\uparrow$       & PC $\uparrow$     &IP $\uparrow$      & \multicolumn{2}{c}{PC $\uparrow$}     \\
		\bottomrule
            ELITE (zero-shot) &                  & 0.228             & 0.146   &-      & -         \\
		Dreambooth  &               & 0.273             & 0.239   &-      & -         \\
	     Custom-Diffusion &       & 0.434             & 0.233    &-     & -     \\
        Fastcomposer &    $\checkmark$        & 0.514             & 0.243      &0.461   &0.235     \\
		
        Subject-Diffusion & $\checkmark$ & 0.605             & 0.228   &0.432      & 0.205     \\
		
            Face-Diffuser &       $\checkmark$       & 0.708     & 0.325        & 0.593         & 0.319     \\
		\bottomrule
          Mixture-of-Attention &     $\checkmark$          & 0.555   & 0.202        & -         & \multicolumn{2}{c}{ - }     \\
  
	\end{tabular} \\
	\label{table:comparison}
\end{table}



==> table/comparison_ss.tex <==
\begin{table}[H]  \centering
	\small
	\caption{Quantitative results for all competing methods on single- and multi-subject generation. IP denotes identity preservation and PC denotes prompt consistency. OF stands for ``optimization-free'' inference.}
	\vspace{-0.4cm}
	\label{table1}
	\begin{tabular}{cc|cc}
		\bottomrule
		\multirow{2}{*}{\textbf{Methods}} & & \multicolumn{2}{c|}{\textit{\textbf{Single-Subject}}} \\
		& OF & IP  $\uparrow$       & PC $\uparrow$       \\
		\bottomrule
            ELITE (zero-shot) &                  & 0.228             & 0.146        \\
		Dreambooth  &               & 0.273             & 0.239       \\
	     Custom-Diffusion &       & 0.434             & 0.233   \\
        Fastcomposer &    $\checkmark$        & 0.514             & 0.243     \\
		
        Subject-Diffusion & $\checkmark$ & 0.605             & 0.228    \\
		
            Face-Diffuser &       $\checkmark$       & 0.708     & 0.325   \\
		% \bottomrule
          Mixture-of-Attention &     $\checkmark$          & 0.555   & 0.202          \\
  
	\end{tabular} \\
	\label{table:comparison}
\end{table}

==> table/related_work.tex <==
% \begin{table}[t]
% \small
% \caption{Comparison between personalization approaches.}
% \label{table:related}
% \begin{tabular}{l|cccc}
% \toprule
%  & Prior  & Multi-  & Optimizat- & Control \\
%   & Preserving & Subject  & ion-Free & -Free \\
% \midrule
% Textual Inversion & $\checkmark$ & & & $\checkmark$ \\
% Dreambooth & & & & $\checkmark$ \\

% Custom Diffusion & & $\checkmark$ & & $\checkmark$ \\
% Modular Customization & & $\checkmark$ & & $\checkmark$ \\
% Mix-of-Show &  & $\checkmark$ & & \\
% IP-Adapter* & $\checkmark$  & $\checkmark$ & $\checkmark$ &  \\
% InstantID & $\checkmark$ & $\checkmark$ & $\checkmark$ & \\
% Fastcomposer & & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
% MoA (Ours) & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[t]
\small
\kcwqa{
\caption{Comparison between personalization approaches. \kac{Some comments to discuss: (1) DB, CD, MC, Mix-of-Show also represent "subject as a token", namely, "a [v] dog", so we have to define what it means.}
% \kac{(2) Modular customization requires spatial-masks, otherwise it doesn't work, so I don't think it's control-free.}
}
\label{table:related}
\begin{tabular}{l|cccc}
\toprule
 & Subject as  & Multi-  & Optimizat- & Layout \\
  & Text Token & Subject  & ion-Free & -Free \\
\midrule
Textual Inversion & $\checkmark$ & & & $\checkmark$ \\
Dreambooth & & & & $\checkmark$ \\

Custom Diffusion & & $\checkmark$ & & $\checkmark$ \\
Modular Customization & & $\checkmark$ & & \\
Mix-of-Show &  & $\checkmark$ & & \\
IP-Adapter &   &  & $\checkmark$ & $\checkmark$ \\
InstantID &  & $\checkmark$ & $\checkmark$ & \\
Fastcomposer & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
MoA (Ours) & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
\bottomrule
\end{tabular}
}
\end{table}
